Coalitional Permutation Manipulations in the Gale-Shapley Algorithm

In this paper, we consider permutation manipulations by any subset of women in the men-proposing version of the Gale-Shapley algorithm. This paper is motivated by the college admissions process in China. Our results also answer an open problem on what can be achieved by permutation manipulations. We present an efficient algorithm to find a strategy profile such that the induced matching is stable and Pareto-optimal (in the set of all achievable stable matchings) while the strategy profile itself is inconspicuous. Surprisingly, we show that such a strategy profile actually forms a Nash equilibrium of the manipulation game. In the end, we show that it is NP-complete to find a manipulation that is strictly better for all members of the coalition. This result demonstrates a sharp contrast between weakly better off outcomes and strictly better-off outcomes.

==> feasibility.tex <==
\section{Feasibility Condition}\label{sec:feasibility}

The concepts of strong Nash equilibria and super-strong Nash equilibria are sometimes criticized to be too strong in that they do not exist in many games. Moreover, it is NP-Hard to decide whether a strong Nash equilibrium or a super-strong Nash equilibrium exists or not (Theorem~\ref{thm:permute_hard_without}).  

We consider the following feasibility condition of a manipulation~\cite{incentive, roth2002economist, gale1985ms}:
 
\begin{condition}[Feasibility]\label{assump}
	A coalition manipulation is feasible if and only if the induced matching is stable with respect to the {\em true} preference profile.
\end{condition}

We call a matching {\em feasible} if it is induced by a feasible coalition manipulation. We redefine the SNE and SSNE with the feasibility condition as follows.

\Ynote{
\begin{definition}[Strong Nash equilibrium (SNE) \& Super-strong Nash equilibrium (SSNE) with the feasibility condition]
	A Nash equilibrium is {\em strong}, if no subset of manipulators can jointly manipulate to a matching that is strictly better off for all of them by a feasible coalition manipulation. A Nash equilibrium is {\em super-strong}, if no subset of manipulators can jointly manipulate to a matching that is weakly better off for all and strictly better off for at least one of them by a feasible coalition manipulation.
\end{definition}}

Condition~\ref{assump} weakens the definitions of strong Nash equilibrium and super-strong Nash equilibrium because it restricts possible deviations of agents to those that induce stable matchings with respect to the true preferences. In general, if without the feasibility condition, a strong Nash equilibrium does not always exists, neither does a super-strong Nash equilibrium (see Section~\ref{sec:example_permute_unstable} for details). Even worse, it is NP-Hard to check the existence of these equilibria without the feasibility condition (Theorem~\ref{thm:permute_hard_without}). In fact, Condition~\ref{assump} is a sufficient condition of the existence of strong Nash equilibrium or super-strong Nash equilibrium in the manipulation game, and moreoever, Condition~\ref{assump} enables efficient algorithms to search those equilibria  (Theorem~\ref{theo:main_permutate}). 

Other than technical necessity mentioned above, Condition~\ref{assump} is well-motivated and standard from the stable matching literature. As \citet{roth2002economist} and \citet{incentive} suggest, stability is of great importance for a successful clearinghouse. Empirical evidence shows that most stable mechanisms have succeeded in practice while almost all unstable ones have failed. If the induced matchings were unstable, a manipulation is no longer a Nash equilibrium, thus agents are unlikely to follow and the manipulations fall apart~\cite{gale1985ms}. Such unpredictability makes the unstable matchings less desirable to the manipulators. 
%This is equivalent to what the condition states: unstable matchings yield low payoffs for the agents. 
Therefore, a coalition manipulation to an unstable matching is hard to form and maintain, since the coalition is likely to collapse.

The condition also fits in the context of the initiative exam example mentioned in the introduction: in order for the colleges in the league to settle for an potentially good outcome, the induced matching after manipulation must be stable; or otherwise the colleges will further deviate and the manipulation falls apart.

\begin{definition}[$S_L$-Pareto-optimal matching]
	A feasible matching $\mu$ is $S_L$-Pareto-optimal if there is no feasible matching in which all manipulators are weakly better off than in $\mu$ and at least one manipulator is strictly better off.
\end{definition}

The above definition can be thought of as the standard $S_L$-Pareto-optimality restricted to feasible matchings. 
Let $S_L(P(M), P(W))$ denote the set of all feasible matchings. We sometimes write $S_L$ for short when $(P(M), P(W))$ is clear from the context. Finally, we say a strategy profile is $S_L$-Pareto-optimal when its induced matching is $S_L$-Pareto-optimal.

The $S_L$-Pareto-optimal strategy profiles also enjoy incentive properties.

\begin{theorem} \label{thm:equivalence}
    The set of induced matchings from $S_L$-Pareto-optimal strategy profiles is the same as the set of super-strong Nash equilibrium outcomes.
\end{theorem}

\citet{gonczarowski2013sisterhood} consider the sisterhood between manipulators and non-manipulators, and give the following result. 

\begin{theorem}[\citet{gonczarowski2013sisterhood}]\label{thm:sisterhood}
Given agents' strict preferences over agents of the other sex, and a set of manipulators $L \in W$ are allowed to use general manipulations, if no lying woman is worse off, then (1) No woman is worse off; (2) No man is better off.
\end{theorem}
Since our setting is a special case of theirs, the above theorem applies to our setting.
\begin{proof}[Proof of Theorem \ref{thm:equivalence}]
	We first prove that all super-strong Nash equilibrium outcomes are $S_L$-Pareto-optimal matchings. Assume on the contrary that a matching $\mu$ is induced by a super-strong Nash equilibrium but is not $S_L$-Pareto-optimal. Thus there exists a matching $\mu'\in S_L$ and $\mu'\ne\mu$ such that $\mu'(w)\succeq_w \mu(w), \forall w \in W$ and $\exists w'\in W$ such that $\mu'(w')\succ_{w'}\mu(w')$. It follows that $\mu'(l)=\mu(l), \forall l \in L$ because $\mu$ is induced by a super-strong Nash equilibrium, and thus we cannot have $\mu'(l)\succ_l\mu(l)$. Let $\mathcal{R}_\mu$ and $\mathcal{R}_{\mu'}$ be the corresponding set of rotations to $\mu$ and $\mu'$, respectively. Since $\mu'(w)\succeq_w \mu(w), \forall w \in W$, we have $\mathcal{R}_\mu\subset \mathcal{R}_{\mu'}$ and $\mathcal{R}_{\mu'}\setminus\mathcal{R}_\mu$ is a closed set that still can be eliminated after eliminating $\mathcal{R}_\mu$. Let $R\in Max(\mathcal{R}_{\mu'}\setminus\mathcal{R}_\mu)$. By Lemma~\ref{EliContainLiar}, there exists a manipulator $l$ in $R$. Thus $\mu'(l)\succ \mu(l)$, which contradicts to the fact that $\mu'(l)=\mu(l), \forall l \in L$.
	
	Now we prove that any $S_L$-Pareto-optimal matching can be induced by a super-strong Nash equilibrium. Assume, for purposes of contradiction, that a matching $\mu$ is $S_L$-Pareto-optimal but cannot be induced by a super-strong Nash equilibrium. Thus any preference profile that yields matching $\mu$ is not a super-strong Nash equilibrium. In particular, we let the manipulators use the inconspicuous manipulation defined above. 
	Let $P$ be the true preference profile and $P'$ be the inconspicuous preference profile that would yield matching $\mu \in S_L(P)$. Since $P'$ is not a super-strong Nash equilibrium, there exists a subset $L_s$ of $L$, if jointly misreport another preference profile, can make the induced matching to be $\mu' \in S_L(P)$, such that $\forall l\in L_s, \mu'(l)\succeq_l^{P}\mu(l)$ and $\exists l'\in L_s, \mu'(l')\succ_{l'}^{P} \mu(l')$. Moreover, there exists $w\in W\setminus L_s$, such that $\mu'(w)\prec_w^{P}\mu(w)$, since otherwise we have $\mu'(w)\succeq_w^{P}\mu(w), \forall w\in W$, which contradicts to the $S_L$-Pareto-optimality of $\mu$. Notice that, in inconspicuous preference profile $P'$, we have for all $w \in W$, $m \succ_w^{P'} \mu(w)$ if and only if $m \succ_w^P \mu(w)$ since the order of men ranked higher than $\mu(w)$ in $P'(w)$ is exactly the same as $P(w)$. Therefore, for all $l \in L_s$, $\mu'(l) \succ_l^{P'} \mu(l)$. However, according to Theorem \ref{thm:sisterhood}, since no manipulators are worse off according to $P'$, we have that no women are worse off according to $P'$. Also, for all $w \in W\setminus L_s$, $\mu'(w) \succeq_l^{P'} \mu(w)$ implies $\mu'(w) \succeq_l^{P} \mu(w)$. Thus, $\mu' \succeq_W^P \mu$. A contradiction.
\end{proof}

The above results show that the Gale-Shapley algorithm is vulnerable to coalition manipulation with the feasibility constraints. However, if a manipulation is not costless such that every manipulator must be strictly better off after the manipulation to preserve individual rationality, we show a hardness result:
    \begin{theorem}\label{theo:hardness_better}
        In permutation manipulations with the feasibility constraints, it is NP-complete to find a manipulation such that the induced matching is strictly better off for all manipulators.
    \end{theorem}    
    
    Therefore, when the manipulation is not costless, a manipulation coalition is unlikely to form and the Gale-Shapley algorithm is immune to coalition manipulations.
%\subsubsection{Number of solutions}

	According to Theorem \ref{theo:hardness_better}, one immediate corollary is that the number of different $S_L$-Pareto-optimal matchings cannot be polynomial in the number of men and women. For otherwise, we can enumerate all such matchings by Algorithm \ref{algorithm} to develop a polynomial time algorithm. Actually, there are $2^{\Theta(|M| + |W|)}$ different feasible matchings, which is $S_L$-Pareto-optimal and strictly better off for all manipulators, in the constructed stable matching problem used in the reduction of Theorem \ref{theo:hardness_better} (see Appendix \ref{appendix:num_pareto_optimal_matching} for details). Last but not least, the problem to compute the number of such matchings is \#P-Hard.	

    \begin{theorem}\label{sharp_P}
        In permutation manipulations, it is \#P-Hard to compute the number of feasible matchings, which are $S_L$-Pareto-optimal and strictly better off for all manipulators.    
    \end{theorem}
    The proofs in this subsection are deferred to Appendix~\ref{proof:hardness_better} and ~\ref{proof:sharp_P}.
